Steward: Natural Language Web Automation

Recently, large language models (LLMs) have demonstrated exceptional capabilities in serving as the foundation for AI assistants. One emerging application of LLMs, navigating through websites and interacting with UI elements across various web pages, remains somewhat underexplored. We introduce Steward, a novel LLM-powered web automation tool designed to serve as a cost-effective, scalable, end-to-end solution for automating web interactions. Traditional browser automation frameworks like Selenium, Puppeteer, and Playwright are not scalable for extensive web interaction tasks, such as studying recommendation algorithms on platforms like YouTube and Twitter. These frameworks require manual coding of interactions, limiting their utility in large-scale or dynamic contexts. Steward addresses these limitations by integrating LLM capabilities with browser automation, allowing for natural language-driven interaction with websites. Steward operates by receiving natural language instructions and reactively planning and executing a sequence of actions on websites, looping until completion, making it a practical tool for developers and researchers to use. It achieves high efficiency, completing actions in 8.52 to 10.14 seconds at a cost of $0.028 per action or an average of $0.18 per task, which is further reduced to 4.8 seconds and $0.022 through a caching mechanism. It runs tasks on real websites with a 40% completion success rate. We discuss various design and implementation challenges, including state representation, action sequence selection, system responsiveness, detecting task completion, and caching implementation.

==> FiguresTex/fig_cache.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{Figures/cache.pdf}
    \caption{}
    \label{fig:cache}
\end{figure}

==> FiguresTex/fig_comparison.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.98\columnwidth]{Figures/comparison.png}
    \caption{Intuitive comparison between prior dynamic privacy analysis tools and \name.}
    \label{fig:comparison}
\end{figure}

==> FiguresTex/fig_state.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.7\columnwidth]{Figures/state.pdf}
    \caption{Features used to define a given state of a website.}
    \label{fig:state}
\end{figure}

==> FiguresTex/fig_teaser_analysis.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=.98\textwidth]{Figures/teaser_analysis.png}
    \caption{\name records any changes in network traffic, cookie placement, and local storage over the course of each task, detecting trackers, data collection of personal information, and privacy violations.}
    \label{fig:teaser_analysis}
\end{figure*}

==> FiguresTex/tab_colored_sample.tex <==
\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
\rowcolor[gray]{0.8}
  & \textbf{\OEM{A}} & \textbf{\OEM{B}} & \textbf{\OEM{C}} & \textbf{\OEM{D}} \\ \hline
\cellcolor{red!30}A & 1600  & 62      & 8    & 22        \\ \hline
\cellcolor{orange!30}B & 1698  & 20      & 11     & 1       \\ \hline
\cellcolor{yellow!30}C & 1076  & 9     & 0       & 1        \\ \hline
\cellcolor{green!30}D & 72    & 45    & 0      & 0         \\ \hline
\cellcolor{blue!30}E & 1107  & 74    & 0      & 0         \\ \hline
\cellcolor{purple!30}F & 780   & 44    & 16     & 16        \\ \hline
\end{tabular}
\caption{OEM VHAL Property occurrences by category}
\label{your-label}
\end{table}

\begin{table}[]
\centering
\begin{tabular}{
  |>{\columncolor[RGB]{255,200,200}}l|
   >{\columncolor[RGB]{255,200,200}}l|
   >{\columncolor[RGB]{255,165,0}}l|
   >{\columncolor[RGB]{255,255,0}}l|
   >{\columncolor[RGB]{0,128,0}}l|
   >{\columncolor[RGB]{0,0,255}}l|
   >{\columncolor[RGB]{128,0,128}}l|
}
\hline
\rowcolor[gray]{0.8}
\textbf{Category} & \textbf{OEM A} & \textbf{OEM B} & \textbf{OEM C} & \textbf{OEM D} \\ \hline
User Pref.        & 1600           & 62             & 8              & 22            \\ \hline
Drive Assist.     & 1698           & 20             & 11             & 1             \\ \hline
Energy            & 1076           & 9              & 0              & 1             \\ \hline
Lighting          & 72             & 45             & 0              & 0             \\ \hline
Diagnosis         & 1107           & 74             & 0              & 0             \\ \hline
Climate           & 780            & 44             & 16             & 16            \\ \hline
\end{tabular}
\caption{Total Custom VHAL Property occurrences in an OEM emulator by category}
\label{your-label}
\end{table}

==> FiguresTex/tab_end_to_end_component.tex <==
\begin{table*}[t]
\caption{End-to-End Component Results}
\begin{center}
\scalebox{0.7}{
  \begin{tabular}{c|c|c|c|c|c|c|c}
    \toprule
    {Model} & {\bf Element Proposal (Recall@5)} & {\bf Action + Element (F1)} & {\bf Validity (F1)} & {\bf End State (F1)} & {\bf Sec. Parameter (Precision@1)} & {\bf High Level (PPL)} & {\bf Page Context (PPL)} \\ 
    \midrule
    ChatGPT 3.5 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
    ChatGPT 3.5 FT & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
    GPT 4 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
    LLaMA2 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
    CodeLLaMA & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
    \bottomrule
    \end{tabular}
}
\end{center}
\label{table:end_to_end_component}
\end{table*}


==> FiguresTex/tab_mind2web.tex <==
\begin{table*}[t]
\caption{Per-Step Component Results}
\begin{center}
\scalebox{0.7}{
  \begin{tabular}{c|c|c|c|c|c|c}
    \toprule
    {\bf Model} & {\bf Element Proposal (Recall@5)} & {\bf @25} & {\bf Element + Action (Top-1 Acc)} & {\bf Validity Check (Precision)} & {\bf End State Termination (F1)} & {\bf Secondary Param (EM)} \\ 
    \midrule
    {\bf GPT 3.5 Turbo} & \textbf{0.5075} & \textbf{0.7437} & 0.5030 & 0.7525 & 0.4823 & 0.8300 \\
    {\bf GPT 3.5 Turbo FT} & -------- & -------- & 0.7305 & \textbf{0.9192} & \textbf{0.7980} & 0.8350 \\
    {\bf GPT 4} & -------- & -------- & \textbf{0.8144} & 0.7900 & 0.6452 & \textbf{0.8650} \\
    % {\bf LLaMA2} & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
    % {\bf CodeLLaMA} & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
    \bottomrule
    \end{tabular}
}
\end{center}
\label{table:per_step_component}
\end{table*}

==> FiguresTex/tab_runtimes.tex <==
% process_screenshot
% 3.8001234375000195
% get_page_context
% 0.771611020999984
% filter_elements
% 0.6247154585000203
% limit_elements
% 0.4835033540000211
% element_proposal
% 0.9799046459998522
% makes_sense_checking
% 0.9592892295000865
% element_action_selection
% 0.9518744165000328
% end_state
% 0.727052583499983
% text_field
% 0.9496144590000313
% select_option
% 0.6733020414998236

\begin{table*}[t]
    \caption{Average Runtime Per Component}
    \begin{center}
    \scalebox{0.7}{
      \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
        \toprule
        \textbf{Subdomain} & Airlines & Auto & Car Rental & Department & Digital & Event & Fashion & Game & General & Ground & Hotel & Movie & Music & Other & Restaurant & Speciality & Sports \\
        \midrule
        \textbf{Actions per Task} & 9.49 & 9.11 & 9.21 & 5.23 & 6.93 & 5.40 & 7.68 & 3.80 & 9.06 & 7.42 & 7.73 & 4.78 & 5.49 & 6.04 & 5.89 & 6.79 & 3.59 \\
        \bottomrule
        \end{tabular}
    }
    \end{center}
    \label{table:subdomain_action_steps}
    \end{table*}

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.
	       

==> Source/600_Case_Studies.tex <==
\section{Case Studies}

\subsection{Booking and Shopping Websites}


\subsection{Automatically Posting Content}


\subsection{Simulated UI User Testing}


\subsection{Studying Recommendation Algorithms}



==> unused/510_AI_Assistant.tex <==
\section{Case Study: AI Web Assistant} \label{sec:results}

\subsection{Design and Implementation}

We created a ChatGPT API function call system to automatically call \name whenever the user's task required access to internet capabilities. Our API performs the user's desired task on websites and returns a response containing the resulting summary.

\subsection{Evaluation}




==> unused/520_Crawl.tex <==
\section{Case Study: Large-Scale Privacy Analysis} \label{sec:results}

\subsection{Inconsistencies and Violations}



\subsection{Comparison with Random Crawl}




==> unused/530_Prompt_Injection.tex <==
\section{Case Study: Prompt Injection and Hijacking} \label{sec:results}

\subsection{Design}

We tested the feasibility of various prompt injection attacks on LLMs embedded in websites and social media. These black-box prompt injection attacks are crafted to perform two types of attacks: (1) LLM stealing attacks and (2) LLM hijacking attacks. The first attack seeks to glean information from the user by telling \name to post the user's task, last actions, HTML information, sites visited, and/or account information publicly. The second attack hijacks \name via prompt injection to perform some malicious actions like purchasing products for the attacker or subscribing to services using the victim's financial information.

% Whole host of nasty attacks: adding accounts, disabling 2-factor authentication, giving up passwords, framing the victim with fake search histories, sending malicious messages, botnet, real-world negative impacts.

"Scriptjacking" and "Botphishing"

\subsection{Evaluation}

